On the Formal Metatheory of the Pure Type Systems using One-sorted Variable Names and Multiple Substitutions

We develop formal theories of conversion for Church-style lambda-terms with Pi-types in first-order syntax using one-sorted variables names and Stoughton's multiple substitutions. We then formalize the Pure Type Systems along some fundamental metatheoretic properties: weakening, syntactic validity, closure under alpha-conversion and substitution. Finally, we compare our formalization with others related. The whole development has been machine-checked using the Agda system. Our work demonstrates that the mechanization of dependent type theory by using conventional syntax and without identifying alpha-convertible lambda-terms is feasible.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{Chaudhuri, Nantes-Sobrinho (Eds.): International Workshop on Logical\\ Frameworks and Meta-Languages: Theory and Practice (LFMTP 2025) \\
EPTCS 431, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.431.2}{10.4204/EPTCS.431.2}}
\pdfoutput=1

